Solving SDP Faster: A Robust IPM Framework and Efficient Implementation

This paper introduces a new robust interior point method analysis for semidefinite programming (SDP). This new robust analysis can be combined with either logarithmic barrier or hybrid barrier. Under this new framework, we can improve the running time of semidefinite programming (SDP) with variable size $n \times n$ and $m$ constraints up to $\epsilon$ accuracy. We show that for the case $m = \Omega(n^2)$, we can solve SDPs in $m^{\omega}$ time. This suggests solving SDP is nearly as fast as solving the linear system with equal number of variables and constraints. This is the first result that tall dense SDP can be solved in the nearly-optimal running time, and it also improves the state-of-the-art SDP solver [Jiang, Kathuria, Lee, Padmanabhan and Song, FOCS 2020]. In addition to our new IPM analysis, we also propose a number of techniques that might be of further interest, such as, maintaining the inverse of a Kronecker product using lazy updates, a general amortization scheme for positive semidefinite matrices.

==> other.tex <==
\section{A summary of amortization techniques}
In Table~\ref{tab:amortize} we summarize the known amortization techniques of various optimization problems. Our amortized analysis is built upon these techniques.
\begin{table}[!h]
    \centering
    \begin{tabular}{|l|l|l|l|} \hline
        {\bf References} & {\bf Problems} & {\bf Objects} & {\bf Tools} \\ \hline
        \cite{v89_lp} & LP & vector & FMM: $\omega$ \\ \hline
        \cite{cls19} & LP & vector & FMM: $\omega,\alpha$ \\ \hline 
        \cite{lsz19} & ERM & block diagonal matrix & FMM: $\omega,\alpha$\\ \hline
        \cite{jlsw20} & CPM & vector & FMM: $\omega,\alpha,\beta,\gamma$ \\ \hline
        \cite{jswz21} & LP & vector & FMM: $\omega,\alpha$ \\ \hline
        \cite{jklps20} & SDP & PSD matrix & FMM: $\omega(\cdot),\alpha$ \\ \hline
        \cite{clp+21} & DNN & multiple vectors & LSH \\ \hline
    \end{tabular}
    \caption{A summary of amortization techniques. FMM denotes Fast matrix multiplication. LP denotes linear programming, SDP denotes semidefinite programming, CPM denotes cutting plane method, ERM denotes empirical risk minization, DNN denotes deep neural networks. We define $\omega, \alpha, \beta, \gamma$ as follows: $n^{\omega+o(1)} = \Tmat(n,n,n)$ \cite{l14}, $n^{2+o(1)} = \Tmat(n,n,n^{\alpha})$ \cite{gu18}, $n^{2} \poly(\log n) = \Tmat(n,n,n^{\beta})$ \cite{c82}, $O(n^2) = \Tmat(n,n,n^{\gamma})$ \cite{bd76}. Further we define $\omega (\cdot)$ function as $n^{\omega(k)+o(1)} = \Tmat(n,n,n^k)$. It is obvious that $\omega(1) = \omega$ and $\omega(\alpha) = 2$. LSH denotes locality sensitive hashing \cite{im98}.}
    \label{tab:amortize}
\end{table}


The first few lines in the table show the amortization of vectors and block diagonal matrices. The amortization technique in \cite{v89_lp} for LP is very simple, and it basically re-computes everything in $n^{0.4}$ iterations. \cite{cls19} proposed a more complicated amortization technique and reduced the amortized time to $n^{\omega-1/2}+n^{2-\alpha/2}$. Later, many work have successfully generalized it to other settings, e.g., ERM \cite{lsz19}, CPM \cite{jlsw20} and DNN \cite{clp+21}. In \cite{jswz21}, the authors proposed a multiple-level amortization technique which improves by a polynomial factor from the one-level amortization used in \cite{cls19}. 

Semidefinite programming considers PSD matrices instead of vectors. The amortization technique in \cite{jklps20} extends several results from \cite{cls19}. However, their amortized cost is still dominated by $m^\omega$, and it was believed to be hard or impossible to have a stronger version of amortization for SDP. That is one of the major obstacles that \cite{jklps20} didn't obtain the optimal running time (see the previously described Bottleneck 2). In this work, we overcome that obstacle. 

==> sketch.tex <==
\section{Sketching}

We can use coordinate-wise embedding property

Let $R \in \R^{b \times n}$ denote the sketching matrix


\subsection{Coordinate wise embedding}

We define coordinate-wise embedding as follows
\begin{definition}[$(\alpha,\beta,\delta)$-coordinate wise embedding]
We say a randomized matrix $R \in \R^{b \times n}$ satisfying $(\alpha,\beta,\delta)$-coordinate wise embedding if
\begin{align*}
1. & ~ \E_{ R \sim \Pi } [ g^\top R^\top R h ] = g^\top h, \\
2. & ~ \E_{ R \sim \Pi } [ ( g^\top R^\top R h )^2 ] \leq (g^\top h)^2 + \frac{\alpha}{b} \|g\|_2^2 \| h \|_2^2, \\
3. & ~ \Pr_{ R \sim \Pi } \left[ | g^\top R^\top R h  - g^\top h  | \geq \frac{\beta}{ \sqrt{b} } \| g \|_2 \| h \|_2 \right] \leq \delta.
\end{align*}
\end{definition}
\begin{remark}
Given a randomized matrix $R \in \R^{b \times n}$ satisfying $(\alpha,\beta,\delta)$-coordinate wise embedding and any orthogonal projection $P\in\R^{n\times n}$, above definition implies
\begin{align*}
1. & ~ \E_{ R \sim \Pi } [ P R^\top R h ] = Ph, \\
2. & ~ \E_{ R \sim \Pi } [ ( P R^\top R h )_i^2 ] \leq (P h)_i^2 + \frac{\alpha}{b} \| h \|_2^2, \\
3. & ~ \Pr_{ R \sim \Pi } \left[ | ( P R^\top R h )_i - ( P h )_i | \geq \frac{\beta}{ \sqrt{b} } \| h \|_2 \right] \leq \delta.
\end{align*}
since $\|P\|_2 \leq 1$ implies $\|P_{i,:}\|_2 \leq 1$ for all $i\in[n]$.
\end{remark}

